Distributed Semantic Segmentation With Improved Rate-Distortion Trade-Off

Distributed deep neural networks (DNNs) for dense perception tasks such as semantic segmentation execute an encoder DNN on edge devices, and a decoder DNN typically on a large-scale cloud platform with a particular constraint on transmission bitrate. Recent works employ source codecs to enable bitrate-efficient transmission between the edge device and the cloud. However, as these approaches are typically bound to a particular type of source codec and alternative network architectures are often not explored, this results in a suboptimal rate-distortion (RD) trade-off in the low-bitrate regime. In this work, we propose two novel source codecs that \textit{enable extremely low bitrates, while improving RD performance}. We demonstrate the effectiveness of our proposed source codecs by achieving state-of-the-art performance in distributed semantic segmentation at below 0.2 (0.03) bits per pixel, measured using the mean intersection-over-union metric on ADE20K (Cityscapes).

==> Figures/latent_block.tex <==
\usetikzlibrary{shapes.geometric, arrows.meta, calc,backgrounds}

\definecolor{encoder_decoder}{RGB}{213, 232, 212}
\definecolor{rectangle}{RGB}{255, 245, 204}
\definecolor{bottleneck_color}{RGB}{230, 221, 184}
\definecolor{_decoder}{RGB}{255, 204, 255} 
\definecolor{conv}{RGB}{255, 255, 255}
%\definecolor{quant_color}{RGB}{255, 162, 234}
\definecolor{quant_color}{RGB}{232, 123, 142}
\definecolor{ae_color}{RGB}{221, 221, 221}
\definecolor{_rectangle}{RGB}{221, 221, 221}
\definecolor{source_color}{RGB}{200, 201, 164}
\definecolor{lsd_color}{RGB}{144, 255, 193}
\definecolor{hyper_color}{RGB}{189, 230, 241}
\definecolor{ce_color}{RGB}{230, 221, 184}
\definecolor{hyperprior_block_color}{RGB}{209, 231,184}

\tikzstyle{encoder} = [trapezium,
    trapezium angle=55,
    trapezium stretches=true,
    minimum width=7.95cm,
    minimum height=5.2cm,
    trapezium right angle=90,
    trapezium left angle=90,
    shape border rotate=180,
    text centered,
    ]

\tikzstyle{hyper_encoder} = [trapezium,
    trapezium angle=55,
    trapezium stretches=true,
    minimum width=2cm,
    minimum height=1.2cm,
    trapezium right angle=70,
    trapezium left angle=70,
    line width=1pt,
    shape border rotate=180,
    text centered,
    draw=black]
\tikzstyle{process} = [rectangle,minimum width=5cm, minimum height=1cm, text
centered, draw=black, text=black,line width = 1pt, fill=conv]
 \tikzstyle{arrow} = [-Triangle, line width=1pt]
 \tikzstyle{label} = [text width= 0.2cm, align=center]
 \tikzstyle{waypoint}=[fill,circle,minimum size=3.5pt,inner sep=0pt]

\begin{tikzpicture} [node distance = 1.5cm,font=\fontsize{16.5}{18.5}\selectfont]

\node (latent_block) [encoder ,minimum width=6.1cm, minimum height=4.3cm, xshift=-4cm, yshift=-0.35cm,  fill=hyperprior_block_color] at (0,0) { } ;

 \node (heading) [xshift=0.25cm,yshift=-0.65cm] at (latent_block.north west)  {\shortstack{\textbf{Latent} \\ [0.05em] \!\!\!\textbf{Block}}  };

%\node (hb_ad) [draw, rectangle, text=black, minimum width=1.55cm, minimum height=1.17cm,  line width=1.5pt,draw=black, fill=ae_color,yshift=0.85cm,xshift=-1.52cm] at (hyperprior_block.south)    {$\mathbf{AD^{\mathcal{H}}}$};

\node (latent_decoder) [draw, hyper_encoder, text=black, minimum width=2.5cm, minimum height=1.17cm,   line width=1.5pt,draw=black, fill=lsd_color,xshift=-1.55cm,yshift=0.8cm] at (latent_block.south)   {$\mathbf{LSD}$};

\node (latent_mean_decoder) [draw, hyper_encoder, text=black, minimum width=2.5cm, minimum height=1.17cm,   line width=1.5pt,draw=black, fill=lsd_color,xshift=1.6cm,yshift=0.0cm,right of=latent_decoder]   {$\mathbf{LMD}$};

\node (concat) [process, xshift=0cm, yshift=0.7cm, minimum width=2.3cm, minimum height=0.8cm,  line width=1.5pt  ,above of=latent_mean_decoder]   {  \text{Concat} };

\draw[arrow] ($([xshift=0cm]latent_decoder.south)+(0,-0.95cm)$)  to node[midway, right,xshift=0.1cm, yshift=-0.12cm,font=\LARGE] {$\boldsymbol{\sigma}^{(n)}$}  (latent_decoder.south);

\draw[arrow] ($([xshift=0cm]latent_mean_decoder.south)+(0,-0.95cm)$)  to node[midway, right,xshift=0.1cm, yshift=-0.12cm,font=\LARGE] {$\boldsymbol{\mu}^{(n)}$}  (latent_mean_decoder.south);

\draw[arrow] (latent_mean_decoder)  to node[midway, right,xshift=0.1cm, yshift=-0.01cm,font=\LARGE] {$\boldsymbol{\mu}^{(n^{\prime})}$}  (concat);

\draw[arrow] (latent_decoder)  to node[midway, right,xshift=0.1cm, yshift=-0.15cm,font=\LARGE] {$\boldsymbol{\sigma}^{(n^{\prime})}$} ++(0,2.2)   --    (concat);

 \draw[arrow] (concat)  to node[midway, right, xshift=0.1cm, yshift=0.47cm, font=\LARGE]  {$\mathbf{a}^{(n)}$} ($([xshift=0cm]concat)+(0,2.05cm)$); 


\end{tikzpicture}

==> ade20k.tex <==
% \documentclass{standalone}

% \usepackage{graphicx,amsmath} % Required for inserting images
% \usepackage[utf8]{inputenc}
% \usepackage{tikz,pgfplots}

\pgfplotsset{compat=1.10}
\usepgfplotslibrary{fillbetween}

\usetikzlibrary{shapes.geometric, arrows.meta, calc, backgrounds}

%\begin{document}

\begin{tikzpicture}

\definecolor{darkgoldenrod1811370}{RGB}{181,137,0}
\definecolor{darkgreen}{RGB}{0,100,0}
\definecolor{lightgray}{RGB}{211,211,211}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{rosybrown163154141}{RGB}{163,154,141}
\definecolor{voilet}{RGB}{139,69,19}
\begin{axis}[
width=12cm,   % Set the width of the plot
height=11cm,
name = bpp_vs_miou,
legend cell align={left},
legend cell align={left},
legend cell align={left},
scaled ticks=false,
tick align=outside,
tick pos=left,
xtick distance=0.2,
tick label style={font=\LARGE},
label style={font=\LARGE},
%x grid style={lightgray},
xlabel={bits per pixel (bpp) },
xmajorgrids,
xmin=0.05, xmax=0.5,
xtick style={color=black},
x tick label style={/pgf/number format/precision=10},
%y grid style={lightgray},
x grid style={gray!50, line width=1.25pt},
y grid style={gray!50, line width=1.25pt},
ylabel={\(\displaystyle \textrm{mIoU}\) (\%)},
ylabel style={yshift=-3pt},
xlabel style={yshift=4pt},
ymajorgrids,
ymin=30, ymax=33.8,
ytick style={color=black},
ytick={30,31,32,33},
yticklabels={
  \(\displaystyle 30\),
  \(\displaystyle 31\),
  \(\displaystyle 32\),
  \(\displaystyle 33\),
}
]

\addplot [
 name path=litcm,
 line width=1.5pt,
 green,
 mark=star,
 mark size=5,
 mark options={ line width=1.7, solid}
 ]
table [y ] {
x    y     
0.08 31.0  
0.12 32.7 
0.18 33.3 
};
\label{litcm_mitb0_ade20k}

\addplot [
name path=ours,
line width=1.5pt,
green,
mark=square,
mark size=3.5,
mark options={ line width=1.7, solid}
]
table [y ] {
x    y     
0.21 30.1   
0.27 32     
0.37 32.8  
0.45 33.7    
};
\label{ours_mitb0_ade20k}

\path[name path=litcm_horiz]
 (axis cs:0.08,31.0) -- (axis cs:0.24,31.0);

\path[name path=ours_vertical]
 (axis cs:0.545,34.8 ) -- (axis cs:0.87,34.8);


% \path [fill=orange!90, fill opacity=0.2] 
% % bottom-left horizontal
% (axis cs:0.08,31.0) -- (axis cs:0.24,31.0) 
% % up along "ours" curve (increasing x)
% -- (axis cs:0.27,32) 
% -- (axis cs:0.37,32.8) 
% -- (axis cs:0.45,33.7) 
% -- (axis cs:0.6,34.1)
% -- (axis cs:0.87,34.8)
% % back along "litcm" curve (decreasing x)
% -- (axis cs:0.541,34.8) 
% -- (axis cs:0.44,34.5) 
% -- (axis cs:0.18,33.3) 
% -- (axis cs:0.12,32.7) 
% -- cycle;

\path [fill=orange!90, fill opacity=0.2] 
% bottom-left horizontal
(axis cs:0.08,31.0) -- (axis cs:0.24,31.0) 
% up along "ours" curve (increasing x)
-- (axis cs:0.27,32) 
-- (axis cs:0.37,32.8) 
-- (axis cs:0.45,33.7) 
% back along "litcm" curve (decreasing x)
-- (axis cs:0.18,33.3) 
-- (axis cs:0.12,32.7) 
-- cycle;

% \draw[dashed, line width=1.7pt]
%   (axis cs:0.08,31.0) -- (axis cs:0.24,31.0);

% \draw[dashed, line width=1.7pt]
%    (axis cs:0.541,34.8) -- (axis cs:0.87,34.8);

%fake plots for the legends
\addplot [line width=1.5pt, gray , dashed]
table {%
1.00 44
};
\label{No_Compression_fake_legend_ade20k}

\addplot [line width=1.5pt,black,mark=star, mark size=5,  mark options={ line width=1.7, solid}]
table {%
1 34.8000030517578
};
\label{Ahuja_fake_legend_ade20k}

\addplot [line width=1.5pt,black,mark=triangle, mark size=5,  mark options={ line width=1.7, solid}]
table {%
1 34.8000030517578
};
\label{Ahuja_fake_legend_ade20k2}

\addplot [line width=1.5pt,black,mark=o, mark size=3.7,  mark options={ line width=1.7, solid}]
table {%
1 34.8000030517578
};
\label{Ahuja_fake_legend_ade20k3}


\addplot [line width=1.5pt,black,mark=square, mark size=3.5,  mark options={ line width=1.7, solid}]
table {%
1 34.8000030517578
};
\label{ours_fake_legend}

\addplot [line width=1.5pt,  red]
table {%
0.4 34 
};
\label{ours_fake_legend_ade20k}

\addplot [line width=1.5pt,  green]
table {%
0.4 34 
};
\label{mit-b0}

\end{axis}

\node (r_1) [draw=none,fill=none,font=\fontsize{15.6}{17.6}\selectfont] at  ([xshift=-1.4cm,yshift=1.4cm]bpp_vs_miou){\shortstack[l]{
     {\textcolor{red}{\textbf{BD-rate}=$-57.2\%$}}
   }};

\node [draw,fill=white,font=\fontsize{14.8}{16.8}\selectfont] at (rel axis cs:0.71,0.13) {
  \shortstack[l]{
   \hspace*{0mm}\textbf{Source codec method}\\
    \ref*{Ahuja_fake_legend_ade20k} \hspace{-0.01em}\textsf{AR-HSM (\textbf{Ours})} \\
    \ref*{ours_fake_legend} \textsf{HS Baseline} \cite{nazir2025efficient}
  }
};
 \end{tikzpicture}

%\end{document}
